FogStore: Toward a Distributed Data Store for Fog Computing

Stateful applications and virtualized network functions (VNFs) can benefit from state externalization to increase their reliability, scalability, and inter-operability. To keep and share the externalized state, distributed data stores (DDSs) are a powerful tool allowing for the management of classical trade-offs in consistency, availability and partitioning tolerance. With the advent of Fog and Edge Computing, stateful applications and VNFs are pushed from the data centers toward the network edge. This poses new challenges on DDSs that are tailored to a deployment in Cloud data centers. In this paper, we propose two novel design goals for DDSs that are tailored to Fog Computing: (1) Fog-aware replica placement, and (2) context-sensitive differential consistency. To realize those design goals on top of existing DDSs, we propose the FogStore system. FogStore manages the needed adaptations in replica placement and consistency management transparently, so that existing DDSs can be plugged into the system. To show the benefits of FogStore, we perform a set of evaluations using the Yahoo Cloud Serving Benchmark.

==> content/notes.tex <==
Note: We require the data store at least to support the CRUD operations (Create, Read, Update and Delete)

Differences between Fog Data Stores and Cloud Data Stores

(1) Placement of replicas

Proposition: In Fog as we view it, we do not have large data centers with racks that capture many nodes, but rather small Fog nodes that are deployed on the network edge. Single Fog nodes do not have high load; different from cloud data center, there are many small nodes. Such can be single servers locally deployed, e.g., in smart homes and smart cities, routers, micro-computers, end users devices.
To keep latency for writes and reads low, the locality of nodes (latency between nodes) should get a strong weight in choosing the placement for replicas of a given data set. The data set should be placed near its location, and not go "to the cloud" or remote Fog nodes; else, the latency benefits of Fog would be lost (when consistency is important).
Claim: None of the current distributed data storage system supports latency-aware replica placements. They are all optimized toward classical data centers and provide rack-aware placement. That is, placement such that data survives the failure of a complete server rack. The assumption is that all nodes in the same data center are "close"any way, providing low communication latency; hence, latency is not explicitly taken into account in placement strategies.


Conclusion: We need to define suitable replica placement strategies for Fog (can not be configured by a "Fog administrator" for every application --- Fog is also way too dynamic for manual configurations)

Evaluations: 
We show that with a simple latency-optimized placement on a fixed topology, the same queries are faster than with naive placement. (Rack-aware placement is not possible as there are no racks).
We might be able to do that by manually configuring a "data center" that comprises the optimal Fog nodes in Cassandra. Or we use a different data store for this experiment that is easy to configure (there are plenty to choose from); MongoDB could also be a good choice.

We can consider using the Yahoo Cloud Serving Benchmark for the comparisons. 


(2) Differentiated Consistency Levels
Proposition: In Fog computing applications, also in Virtualized Network Functions, the data stored in a distributed data store can have different consistency requirements for (a) different users using the same data, (b) the same users using the same data, but from different locations (example: car reading the traffic light from close or from far away; close: consistency important as not to crash with other cars, far away: consistency not important, traffic light switching only used for optimizing speeding to save fuel).

Claim: Classical cloud data stores would provide the same consistency guarantees for all users of the same data, no matter of the type of application and the location of user and data. 

Both points, (1) and (2) come from the fact that in cloud, the locality of data and users is not considered / constrained. Everything is considered global-scale. The strong point for Fog comes with regional-scale use cases. Regional use cases demand for regional data storage solutions (close to edge, not in data center).




Conclusion:

Evaluations:
A simple setup where local and remote users write and read local data sets (that are placed in data store nodes close to the data). Two setups: Everybody does consistent reads. Or: Local users do consistent reads (at least quorum), remote users do one-shot reads. We can use Cassandra as the system here, because it allows for per-operation consistency specification.


Overall conclusion: Pointing out that some data stores already bring configuration options that would allow them for being made Fog-enabled. However, the setup of the system should be automatically set and adapted to the data, which will require some conceptual developments. Furthermore, none of the systems brings all that is necessary to be Fog-configured; we found useful parts scattered among the different systems. Our micro benchmarks show that implementing the Fog-friendly behavior promises to boost performance for Fog deployments. Some of the ingredients are already there. Others have to be developed. And a data store needs to be compiled that puts all the stuff together, such that setup is easy to use for Fog (FogStore API).


There are further points that could be worth looking into. 
- Scaling with many nodes. Fog is (a) less reliable, (b) best when pushed to the edge as far as possible. This might require that more nodes are installed than in traditional setups. The question is how existing systems scale with more nodes (as they often use gossiping). And how would they scale with more data replicas (this will, however, always stay a conceptual problem). We can use this point just as a pointer to future work; it might be a minor point, and also might be solved differently (e.g., by using different installments of data stores for different regions, and a high-level router, in case that remote data is queried). Hence, the problem itself might not be something solved on the level of data store.

----


Maybe rewrite the storyline a bit. 

Many applications and VNFs are stateful
State externalization can be good for two reasons:
- Reliability / Failure recovery / resilience
- Sharing state among multiple instances of the same application or among multiple different applications
To externalize, reliably store, and share data, distributed data stores are a widely applicable solution.
In Fog Computing, reliability and state sharing face new design goals. Replica placement, and differential consistency. (a) important for fault tolerance, and also to have good write and read latency, (b) important, as the consistency needed on the data can be different among multiple instances of the same application because of the application instance's context; and among multiple different applications due to the different applications different purposes what to do with the data,

